Auto-BI: Automatically Build BI-Models Leveraging Local Join Prediction and Global Schema Graph

Business Intelligence (BI) is crucial in modern enterprises and billion-dollar business. Traditionally, technical experts like database administrators would manually prepare BI-models (e.g., in star or snowflake schemas) that join tables in data warehouses, before less-technical business users can run analytics using end-user dashboarding tools. However, the popularity of self-service BI (e.g., Tableau and Power-BI) in recent years creates a strong demand for less technical end-users to build BI-models themselves. We develop an Auto-BI system that can accurately predict BI models given a set of input tables, using a principled graph-based optimization problem we propose called \textit{k-Min-Cost-Arborescence} (k-MCA), which holistically considers both local join prediction and global schema-graph structures, leveraging a graph-theoretical structure called \textit{arborescence}. While we prove k-MCA is intractable and inapproximate in general, we develop novel algorithms that can solve k-MCA optimally, which is shown to be efficient in practice with sub-second latency and can scale to the largest BI-models we encounter (with close to 100 tables). Auto-BI is rigorously evaluated on a unique dataset with over 100K real BI models we harvested, as well as on 4 popular TPC benchmarks. It is shown to be both efficient and accurate, achieving over 0.9 F1-score on both real and synthetic benchmarks.

==> apx-ablation.tex <==

\section{Details on ablation study}
\label{apx:ablation}


%\underline{The effect of k-MCA formulation.}  any subgraph that can maximizes prob. 
We perform an ablation study to analyze the benefits of various ideas developed in \abi, using the 1000-case \textsc{Real} benchmark. Our results are summarized in Figure~\ref{fig:ablation}.


\noindent\underline{The effect of FK-once constraint.} The bar marked as  ``\textsf{no-FK-once-constraint}'' in Figure~\ref{fig:ablation} shows the result quality that removes the FK-once constraint (or using k-MCA instead of k-MCA-CC). %FK-once refers to the constraint that one FK cannot link to multiple PKs, which is adopted in several previous works~\cite{chen2014fast,hpi}.
There is a noticeable drop in precision/recall, showing the importance of this constraint in k-MCA-CC.
%If we remove this constraint, the edge precision, recall, F-1 and case precision is 0.02, 0.01,  0.02 and 0.02 worse than \abi, respectively. We can draw the conclusion that FK-once is a valid constraint but will not make a huge difference. 

\noindent\underline{The effect of precision-mode.} The  ``\textsf{no-precision-mode}'' bar shows the result quality if we omit the precision-mode step (Section~\ref{subsec:abi-p}) and use the recall-mode directly (Section~\ref{subsec:abi-r}). We see a substantial drop in precision (6 and 13 percentage points at edge-level and case-level, respectively), again showing the importance of k-MCA-CC.% to find the backbones of the underlying schema graphs. 

%If we skip precision mode k-MCA and directly run the recall-mode k-MCA, we observe performance degrades for edge precision and case precision by 0.06 and 0.13, respectively, which demonstrates that the precision-mode k-MCA can capture the desired k-MCA graph structure effectively and thus have a great improvement for edge precision and case precision. Without the precision-mode k-MCA being running, only picking valid edges with high scores as recall-mode k-MCA is difficult to get the desired performance. 

\noindent\underline{The effect of N-1/1-1 separation in local classifier.} The ``\textsf{no-N-1/1-1-seperation}'' bar in Figure~\ref{fig:ablation} shows the results when we use one local classifier, instead of splitting N-1 and 1-1 joins into two prediction tasks (Section~\ref{subsec:local-join}). The drop in quality is evident, showing the benefit of this optimization.
%\abi separates N-1 and 1-1 edges. If we merge them together and use the features of N-1 edges, the edge precision, recall, F-1 and case precision are all around 0.03 worse than \abi. This demonstrates that N-1 and 1-1 edges have slight different features and treating them separately would improve the overall quality of the local classifier, and thus improve \abi.  

\noindent\underline{The effect of label transitivity in local classifier.} The bar for ``\textsf{no-label-transitivity}'' shows the drop in quality when we do not apply label transitivity in  local classification  (Section~\ref{subsec:local-join}). The effect is noticeable but somewhat diluted when averaged across 1000-case, as the benefit  is more pronounced on large cases and less obvious on smaller one. %cases with more complex join paths, and less evident on smaller cases with few tables. 
%When we train the local classifier, we enhance labels with transitivity, i.e., increase the number of positive labels from ground truth in BI models using transitive property if two columns are semantically equivalent. Enabling this optimization increases the edge precision, recall and F-1 by 0.01, 0.02, 0.02, and case precision by 0.02.  

\noindent\underline{The effect of no data-value features in local classifier.} The ``\textsf{no-data-features}'' bar shows the effect of removing features relating to data-value in our local classifier (we use meta-data features only instead). This directly corresponds to our lightweight \abi-S (Section~\ref{subsec:exp_overall}). The drop in performance is apparent but not too significant, which gives  us a useful trade-off between quality and latency. %(since \abi-S is 5x more efficient as shown in Figure~\ref{fig:end_to_end_time}). 

%As we can see, removing data features from local classifier leads to the performance down for edge precision, recall, F-1 by 0.04, 0.03, 0.07, and case precision by 0.1. However, \abi-S has superior end to end efficiency, i.e., 0.45 seconds on average for 1000 cases in real BI benchmarks, comparing with other methods as shown in Table~\ref{tab:end_to_end_time}. In the case where the end to end time constraint is tight, \abi-S is acceptable with the sacrifice of accuracy. 

\noindent\underline{The effect of using local classifier only.} The ``\textsf{LC-only}'' bar shows the performance if we  employ the same local classifier at the edge-level (keeping edges that have calibrated probability over 0.5), without using a holistic k-MCA optimization. The difference in performance is significant (25 percentage points in case-precision), showing the importance of k-MCA.
%and we select the candidate column pairs with the probability higher than 0.5 as the output of the local classifier prediction. As we can see, \abi outperforms classifier prediction by 0.1 edge precision, 0.03 edge recall, 0.06 edge F-1 and 0.25 case precision, which demonstrates that leveraging the global k-MCA graph structure is able to greatly help the local predictions. 
% \begin{table}[]
% \small
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     Methods & Metrics & Abl-1 & Abl-2 &  Abl-3 & Abl-4 & Abl-5 \\ \hline
%     \multirow{4}{4em}{\abi-P}& $P_{edge}$ &0.97 & N/A & 0.96 & 0.97 & 0.97 \\ 
%     & $R_{edge}$ &0.69 & N/A& 0.63 &0.66 &  0.65  \\
%     & $F_{edge}$ &0.78 & N/A&0.72 &0.74 & 0.74 \\ 
%     & $P_{case}$ &0.89 & N/A& 0.88 &0.91 & 0.91 \\ \hline
%     \multirow{4}{4em}{\abi}& $P_{edge}$ & 0.96& 0.93 & 0.96 &0.97 & 0.97 \\ 
%     & $R_{edge}$ &0.9 &0.87 & 0.85 & 0.86&  0.86\\ 
%     & $F_{edge}$ &0.92 &0.88 & 0.88 & 0.89& 0.9 \\ 
%     & $P_{case}$ &0.83 &0.69 & 0.82& 0.83&  0.83\\ \hline
%     \end{tabular}
%     \caption{Results of Ablation Studies.   }
%     \vspace{-1em}
%     \label{tab:alation}
% \end{table}

 


% \begin{figure}[tb]
% 	\centering
% %\hspace{-9mm}
% 	\includegraphics[width=0.95\linewidth]{figures/mca_calls_3.eps}
% 	\vspace{-1em}
% 	\caption{Effect of efficiency optimization techniques (measured by the number of 1-MCA calls).} 
% 	\vspace{-1.5em}
% 	\label{fig:efficiency_ablation}
% \end{figure}


% \begin{figure}[tb]
% 	\centering
% %\hspace{-9mm}
% 	\includegraphics[width=0.95\linewidth]{figures/ablation1.eps}
% 	\vspace{-1em}
% 	\caption{Ablation study of \abi on \textsc{Real}. }
% 	\vspace{-1.5em}
% 	\label{fig:ablation}
% \end{figure}


==> apx-advanced-joins.tex <==

\section{Handle Advanced Joins}
\label{apx:advanced-join}

These are important  because we observe in real Power-BI models that users write scripts to perform transformations (e.g., merging columns, split columns, and other string-manipulations) that derive suitable join columns, before they can invoke standard equi-joins. This is obviously not easy for less-technical non-programmer users that we target in \abi. We thus build upon existing transformation-join~\cite{zhu2017auto} to automatically detect and perform such joins.

Similarly, in Power-BI models users also write scripts to replace certain values in one join column (e.g., replacing ``United States'' with ``United States of America''), just so that the modified values can equi-join values from the other join column. We thus leverage existing fuzzy-join~\cite{li2021auto} to also automatically perform fuzzy joins.

\begin{definition}
\label{def:abi}
(\abi). Given a set of input tables $\mathbf{T} = \{T_1, T_2, \ldots T_n\}$, where each table consists of a list of attributes $T_i = (C_{i1}, C_{i2}, \ldots C_{im})$, predict  a BI model $M(\mathbf{T})$ for the given $\mathbf{T}$, where $M(\mathbf{T}) = \{\left( (C_{ij}, C_{ik} \ldots), (C_{lp}, C_{lq} \ldots) \right)\}$ is a set of join relationships that can be equi-join,  transformation-join, or fuzzy-join.
\end{definition}


\subsection{Automate Non-equi-Joins}
\label{subsec:complex-join}

\textbf{Transformation-join}

\textbf{Fuzzy-join}

==> apx-proof-kmca.tex <==
\section{Proof of Theorem 2}
\label{apx:proof-kmca}

\begin{proof}
Given a graph $G=(V, E)$, let $J^*_k$ be the optimal $k$-MCA of $G$, with objective function value $c_k(J^*_k)$ as defined in Equation~\eqref{eqn:kmca_obj}. Because $J^*_k$  is a $k$-arboresence, by Definition~\ref{def:k-arboresence}, $J^*_k$ has exactly $k$ disjoint components $\{G_1, G_2, \ldots G_k\}$, all of which are 1-arboresence, with $R = \{r_1, r_2, \ldots r_k\}$ as their roots.

We show that on our constructed graph $G' = (V', E')$, the solution $J^*_1 = J^*_k \cup \{(r, r_i) | r_i \in [k]\}$ must be an optimal solution to the 1-MCA problem on $G'$.

We show this by contradiction. Suppose $J^*_1$ is not an optimal solution to $G'$, which means that there is another $J'_1$ with a smaller cost as defined in the 1-MCA objective function (Equation~\eqref{eqn:1mca_obj}), written as 
\begin{equation}
\label{eqn:proof_expand_0}
c_1(J'_1) < c_1(J^*_1)
\end{equation}
In the solution $J'_1$, let $R'$ be the set of vertices incident with artificial root $r$. Removing from $J'_1$ the set of edges incident with $r$ produces $J'_k = J'_1 \setminus \{e(r, r') | r' \in R'\}$.  $J'_k$ is an $|R'|$-arboresence, and thus a feasible solution to $k$-MCA on $G$. Similarly, removing from $J^*_1$ the set of edges incident with $r$ produces $J^*_k = J^*_1 \setminus \{e(r, r') | r' \in R\}$, which is also a feasible solution to $k$-MCA on $G$.

Since $J^*_k$ is an $|R|$-arboresence and $J^_k$ is an $|R'|$-arboresence, by the definition of $c_k$ in Equation~\eqref{eqn:kmca_obj}, we know 
\begin{equation}
\label{eqn:obj_expand_1}
c_k(J^*_k) = \sum_{e\in J^*_k}{w(e)} + (|R|-1)p
\end{equation}
\begin{equation}
\label{eqn:obj_expand_2}
c_k(J'_k) = \sum_{e\in J'_k}{w(e)} + (|R'|-1)p
\end{equation}
Because we know $J^*_k$ is an optimal solution to $k$-MCA on $G$, we know $c_k(J^*_k) \leq c_k(J'_k)$. Combining with Equation~\eqref{eqn:obj_expand_1} and Equation~\eqref{eqn:obj_expand_2}, we get  
\begin{equation}
\label{eqn:obj_expand_3}
\sum_{e\in J^*_k}{w(e)} + (|R|-1)p \leq \sum_{e\in J'_k}{w(e)} + (|R'|-1)p
\end{equation}
Adding $p$ to both sides of Equation~\eqref{eqn:obj_expand_3}, we get $\sum_{e\in J^*_k}{w(e)} + (|R|)p \leq \sum_{e\in J'_k}{w(e)} + (|R'|)p$. Note that the left-hand-side is exactly the objective-value of $J^*_1$ on $G'$, or $c_1(J^*_1)$, while the right-hand-side is the  objective-value of $J'_1$ on $G'$. This gives $c_1(J^*_1) \leq c_1(J'_1)$, contradicting with  our assumption in Equation~\eqref{eqn:proof_expand_0}, thus proving that  $J^*_1$ must be an optimal solution to 1-MCA on $G'$, which can be solved optimally in Line~\ref{line:kmca-solve-1mca} of Algorithm~\ref{alg:k-mca}.


Since 1-MCA (Line~\ref{line:kmca-solve-1mca}) is solvable in polynomial time, and all other steps in Algorithm~\ref{alg:k-mca} takes time polynomial in the input size, we conclude that Algorithm~\ref{alg:k-mca}  can solve $k$-MCA optimally, in polynomial time.
\end{proof}

==> architecture.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{System Architecture}

TBD



==> auto-validate-horizontal.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Auto-Validate with Horizontal Cuts}

TBD


